Averages of b-hadron, c-hadron, and tau-lepton Properties

This article reports world averages for measurements of b-hadron, c-hadron, and tau-lepton properties obtained by the Heavy Flavor Averaging Group (HFAG) using results available at least through the end of 2009. Some of the world averages presented use data available through the spring of 2010. For the averaging, common input parameters used in the various analyses are adjusted (rescaled) to common values, and known correlations are taken into account. The averages include branching fractions, lifetimes, neutral meson mixing parameters, CP violation parameters, and parameters of semileptonic decays.

==> Olivier.tex <==
\section{Examples}
here is an example for 63~\cite{CDFNote:8524,*Abulencia:2006dr,*Acosta:2004gt}, and one for 81~\cite{CDFNote:9203}, another for 146~\cite{Quick:note,*Charles:2004jd,*Bona:2006ah}, and for 153~\cite{Okamoto:2005zg,*Gray:2005ad,*Aoki:2003xb}.


==> hfag_refs.tex <==
% Obsolete 
% \begin{thebibliography}{999}
% 
% %-- Introduction
% 
% \bibitem{ref_ckm}
%  N. Cabibbo, Phys. Rev. Lett. 10, 531 (1963);
%  M. Kobayashi and T. Maskawa, Prog. Theor. Phys. {\bf 49}, 652 (1973).
% 
% \bibitem{LEPHFS}
% ALEPH, CDF, DELPHI, L3, OPAL, 
% and SLD collaborations, ``Combined results on \b-hadron 
% production rates and decay properties'',
% CERN-EP-2000-096, hep-ex/0009052 (2000); updated in
% CERN-EP-2001-050, hep-ex/0112028 (2001).
% 
% \bibitem{PDG_2007}
% W.-M. Yao et al., Journal of Physics, G 33, 1 (2006);
% see also 2007 update at {\tt http://pdg.lbl.gov/}.
% 
% \bibitem{hfag_hepex_endof2006}
%  Heavy Flavor Averaging Group (HFAG), ``Averages of $b$-hadron Properties
%  at the End of 2006'' arXiv:0704.3575 (2007).
% 
% %\bibitem{hfag_hepex_winter2005}
% 
% %\bibitem{Eidelman:2004wy}
% % S.~Eidelman {\em et al.}  (Particle Data Group Collaboration),
% % Phys.\ Lett.\ B {\bf 592}, 1 (2004).
% %%CITATION = PHLTA,B592,1;%%
% 
% %\input{life_mix_references.tex}
% 
% %\input{./slbdecays/slb_refs.tex}
% 
% %\input{cp_uta_refs.tex}
% 
% \input{rare/rare_refs.tex}
% 
% %\input{./charm/charm_refs.tex}
% 
% % \end{thebibliography}


==> rare/rare_refs.tex <==

\bibitem {bf} O. Buchm\"uller and H. Fl\"acher, hep-ph/0507253.
\bibitem{cleo} S. Chen \etal\ (CLEO Collaboration), \prl{87}, 251807 (2001).
\bibitem{belle1} K. Abe \etal\ (Belle Collaboration), \plb{511}, 151 (2001).
\bibitem{babar3} BaBar Collaboration (B. Aubert \etal), \prd{77}, 051103 (2008).
\bibitem{babar1} B. Aubert \etal\ (\babar\ Collaboration), \prd{72}, 052004 (2005).
\bibitem{babar2} B. Aubert \etal\ (\babar\ Collaboration), \prl{97}, 171803 (2006).
\bibitem{babar3} B. Aubert \etal\ (\babar\ Collaboration), \prd{77}, 051103 (2008).
\bibitem{belle2} A. Limosani \etal\ (Belle Collaboration), \prl{103}, 241801 (2009).


==> tables/cp_uta/psiphi.tex <==
\begin{table}[htb]
	\begin{center}
		\caption{
			 Results from time-dependent analysis of $\Bs \to J/\psi \phi$.
		}
		\vspace{0.2cm}
		\setlength{\tabcolsep}{0.0pc}
% make this tabular (not tabular*) and resize down to \textwidth
% change @{\extracolsep{\fill}} to @{\extracolsep{2mm}}
    \resizebox{\textwidth}{!}{
      \begin{tabular}{@{\extracolsep{2mm}}lrccccc} 
        \hline
        \mc{2}{l}{Experiment} & $\tau(\Bs)$ & $\Delta\Gamma$ & $\phi_s$ & $A_\perp$ & $|A_0|^2 - |A|_\parallel^2$ \\
	\dzero & \cite{:2008fj} & $1.52 \pm 0.06 \pm 0.01$ & $0.19 \pm 0.07 \,^{+0.02}_{-0.01}$ & $-0.57 \,^{+0.24}_{-0.30} \,^{+0.07}_{-0.02}$ & $0.41 \pm 0.04 \,^{+0.01}_{-0.02}$ & $0.34 \pm 0.05 \pm 0.03$ \\
        \hline
      \end{tabular}
    }

		\label{tab:cp_uta:ccs:psiphi}
	\end{center}
\end{table}




==> tables/slb/dlnu.tex <==
% ----------------------------------------------------------------------0
\begin{table}[!htb]
\caption{Average of the branching fraction $\cbf(\BzbDplnu)$ and individual
results. }
\begin{center}
\begin{tabular}{|l|c|c|}\hline
Experiment                                 &$\cbf(\BzbDplnu) [\%]$ (rescaled) &$\cbf(\BzbDplnu) [\%]$ (published) \\
\hline\hline 
ALEPH ~\hfill\cite{Buskulic:1996yq}        &$2.15 \pm0.18_{\rm stat} \pm0.37_{\rm syst}$  &$2.35 \pm0.18_{\rm stat} \pm0.44_{\rm syst}$ \\
CLEO  ~\hfill\cite{Bartelt:1998dq}         &$2.07 \pm0.13_{\rm stat} \pm0.16_{\rm syst}$  &$2.20 \pm0.13_{\rm stat} \pm0.18_{\rm syst}$ \\
\belle  ~\hfill\cite{Abe:2001yf}           &$2.13 \pm0.12_{\rm stat} \pm0.39_{\rm syst}$  &$2.13 \pm0.12_{\rm stat} \pm0.41_{\rm syst}$ \\
\hline 
{\bf Average}                              &\mathversion{bold}$2.09 \pm0.18$      &\mathversion{bold}$\chi^2/\dof = 0.04/2$ (CL=$98\%$)  \\
\hline 
\end{tabular}
\end{center}
\label{tab:dlnu}
\end{table}
% ----------------------------------------------------------------------


